Machine Learning for Tangible Effects: Natural Language Processing for Uncovering the Illicit Massage Industry & Computer Vision for Tactile Sensing

I explore two questions in this thesis: how can computer science be used to fight human trafficking? And how can computer vision create a sense of touch? I use natural language processing (NLP) to monitor the United States illicit massage industry (IMI), a multi-billion dollar industry that offers not just therapeutic massages but also commercial sexual services. Employees of this industry are often immigrant women with few job opportunities, leaving them vulnerable to fraud, coercion, and other facets of human trafficking. Monitoring spatiotemporal trends helps prevent trafficking in the IMI. By creating datasets with three publicly-accessible websites: Google Places, Rubmaps, and AMPReviews, combined with NLP techniques such as bag-of-words and Word2Vec, I show how to derive insights into the labor pressures and language barriers that employees face, as well as the income, demographics, and societal pressures affecting sex buyers. I include a call-to-action to other researchers given these datasets. I also consider how to creating synthetic financial data, which can aid with counter-trafficking in the banking sector. I use an agent-based model to create both tabular and payee-recipient graph data. I then consider the role of computer vision in making tactile sensors. I report on a novel sensor, the Digger Finger, that adapts the Gelsight sensor to finding objects in granular media. Changes include using a wedge shape to facilitate digging, replacing the internal lighting LEDs with fluorescent paint, and adding a vibrator motor to counteract jamming. Finally, I also show how to use a webcam and a printed reference marker, or fiducial, to create a low-cost six-axis force-torque sensor. This sensor is up to a hundred times less expensive than commercial sensors, allowing for a wider range of applications. For this and earlier chapters I release design files and code as open source.

==> frontmatter/abstract.tex <==


  






I explore two questions in this thesis: how can computer science be used to fight human trafficking? And how can computer vision create a sense of touch?

The United States illicit massage industry (IMI) is a multi-billion dollar industry that offers not just therapeutic massages but also commercial sexual services. Illicit massage parlors number in the thousands and exist in every major city in the United States. Employees are often immigrant women with few job opportunities, leaving them vulnerable to fraud, coercion, and other facets of human trafficking. By creating datasets using three publicly-accessible websites: Google Places, Rubmaps, and the AMPReviews forum, I show how we can use natural language processing tools such as bag-of-words to help monitor spatiotemporal trends in the IMI. Monitoring forms an essential part of preventing trafficking and protecting employees within the IMI. I further show how to use word embeddings such as Word2Vec to derive insights into the labor pressures and language barriers that employees face, as well as the income, demographics, and societal pressures affecting sex buyers. 

I also consider counter-trafficking in the banking sector. Human trafficking is about money, much of which will flow through the legal financial system at one point or another. Thus, banks play a unique role in counter-trafficking and are legally required to have safeguards to guarantee they are not aiding or abetting criminal activity. My preliminary work looks at creating synthetic transaction data so that researchers can more easily prototype, evaluate, and collaborate in advancing the field of analytics in support of anti-money laundering. This work adopts agent-based modeling and is inspired by red-flagged transactional behaviors from the United States and the Canadian financial regulatory agencies. I show both the uses and limitations of my model in generating timestamps and payee-recipient graphs for transactions. 

Finally, I consider the role of computer vision in creating tactile sensors. Tactile sensors are critical for robots that seek to manipulate and interact with the world, a prerequisite for helping with household tasks. Existing sensors the Gelsight sensor, which consists of a camera facing a gel that is lit from multiple angles. The surface of the gel is slightly translucent and slightly reflective (semi-specular). When objects are pressed into the gel, the image can be considered a tactile image. To adapt a Gelsight sensor to the task of finding buried objects in sand, specific modifications include changing the shape of the sensor to a wedge to allow for digging down into the granular media. The novel use of fluorescent paint instead of LEDs for gel lighting allows for significant sensor size reduction. Finally, an integrated vibrator motor counteracts jamming in the granular media, reducing force requirements for moving through the media.


This work also shows how to use a webcam and a printed reference marker, or fiducial, to create a low-cost six-axis force-torque sensor. Commercial six-axis force-torque sensors cost thousands of dollars and often contain delicate strain gauges. By contrast, this sensor is inexpensive, made using readily-available rapid prototyping technologies, and easy to modify.  All code and hardware design files are open sourced, opening up six-axis force-torque sensing to a wider range of applications.

\centerline{Note: Please refer to arXiv for the latest version of this thesis.}



















